Dream machine -- the next creative economy

We examine the structural transformation of creative industries under generative artificial intelligence, drawing on 374 primary sources spanning policy documents, industry data, creator surveys, and platform analytics. Beginning with the December 2024 release of OpenAI's Sora video model as a watershed event, we trace the historical pattern of creative resistance to technological disruption, then develop an analytical framework -- the Human-AI Agency Continuum for mapping the spectrum of human and machine collaboration in creative work. We present evidence for the "slop ceiling," an audience-imposed quality threshold that constrains AI-generated content to approximately 1--3% of platform streams despite comprising 44% of uploads. Analysis of the UK Government's 2025 consultation on AI and copyright (over 11,500 responses, 88% opposing expanded AI training rights) reveals deep structural tensions between technology firms and creative workers. We investigate how major studios, from Disney's $1 billion OpenAI investment to Netflix's AI-native animation unit, are positioning for an AI-augmented production pipeline. The work covers coordination collapse in creative supply chains, the emergence of new professional roles such as prompt engineers and AI orchestrators, and proposes four principles for navigating the transition: transparency, consent, compensation, and human-centred design. Eight appendices provide quantitative analysis, a glossary, topical bibliography, and deep dives into shadow AI adoption, AI stigma, and algorithmic intent.

==> figures/wardley_creative_economy.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{figures/wardley_creative_economy.png}
\caption{The Creative Economy Landscape --- a Wardley map of the broader value chain during AI transition. Upper layer (\emph{visible}): the working creative's outputs, audience relationship, and brand/authenticity signal. Middle layer (\emph{orchestration}): AI tool stack, human judgement, and the emerging attribution infrastructure. Infrastructure layer: foundation models, training data, and compute commoditising toward utility. C2PA/provenance standards occupy the disclosure layer between orchestration and infrastructure. The authenticity premium (upper left) and the slop ceiling (middle right) are the two market forces shaping creative-economy strategy in 2025--26. Based on the analysis in Chapters~\ref{ch:5}, \ref{ch:7}, and \ref{ch:11}.}
\label{fig:wardley-creative-economy}
\end{figure}


==> figures/wardley_studios.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{figures/wardley_studios.png}
\caption{The Four Strategic Positions --- a Wardley map of how studios positioned themselves relative to AI adoption in creative production (October 2025--May 2026). Position~1 (\emph{All-in}): Netflix, Disney, Amazon --- AI integrated across the full production stack. Position~2 (\emph{AI-native}): Imaginae, Wonder, Asteria, Chapter41, Kartel, Obsidian --- built AI-first from inception. Position~3 (\emph{Refusal}): Jagex, Larian, Games Workshop, Hooded Horse, Aardman --- generative AI excluded, human craft preserved as competitive positioning. Position~4 (\emph{The Middle}): Sony, Bethesda --- AI in the workflow, human intent in the finished work. Based on the taxonomy developed in Chapter~\ref{ch:7}.}
\label{fig:wardley-studios}
\end{figure}

